Density Distribution-based Learning Framework for Addressing Online Continual Learning Challenges

In this paper, we address the challenges of online Continual Learning (CL) by introducing a density distribution-based learning framework. CL, especially the Class Incremental Learning, enables adaptation to new test distributions while continuously learning from a single-pass training data stream, which is more in line with the practical application requirements of real-world scenarios. However, existing CL methods often suffer from catastrophic forgetting and higher computing costs due to complex algorithm designs, limiting their practical use. Our proposed framework overcomes these limitations by achieving superior average accuracy and time-space efficiency, bridging the performance gap between CL and classical machine learning. Specifically, we adopt an independent Generative Kernel Density Estimation (GKDE) model for each CL task. During the testing stage, the GKDEs utilize a self-reported max probability density value to determine which one is responsible for predicting incoming test instances. A GKDE-based learning objective can ensure that samples with the same label are grouped together, while dissimilar instances are pushed farther apart. Extensive experiments conducted on multiple CL datasets validate the effectiveness of our proposed framework. Our method outperforms popular CL approaches by a significant margin, while maintaining competitive time-space efficiency, making our framework suitable for real-world applications. Code will be available at https://github.com/xxxx/xxxx.

==> sec/0_abstract1.tex <==
\begin{abstract}
In this paper, we address the challenges of online Continual Learning (CL) by introducing a density distribution-based learning framework. CL enables adaptation to new test distributions while continuously learning from a single-pass training data stream, aligning with practical applications of machine learning methods. However, existing CL methods often suffer from catastrophic forgetting (CF) and higher computing costs due to complex algorithm designs, limiting their practicality compared to classical machine learning paradigms. Our proposed framework overcomes these limitations by achieving superior average accuracy and training efficiency, bridging the performance gap between CL and classical machine learning. Specifically, we adopt an independent Generated Kernel Density Estimation (GKDE) function for each CL task. During the testing stage, the GKDEs utilize a self-reported max probability distance metric to determine which one is responsible for predicting incoming test instances. A GKDE-based learning objective is introduced to ensure that samples with the same label are grouped together, while dissimilar instances are pushed farther apart. Extensive experiments conducted on multiple CL datasets validate the effectiveness of our proposed framework. Our method outperforms popular CL approaches by a significant margin, while maintaining competitive training efficiency and memory usage, making our framework suitable for real-world applications. Code will be available at https://github.com/xxxx/xxxx.
\end{abstract}

==> sec/0_abstract_-_____.tex <==
\begin{abstract}
In this paper, we address the challenges of online Continual Learning (CL) by introducing a density distribution-based learning framework. CL enables adaptation to new test distributions while continuously learning from a single-pass training data stream, especially the Class Incremental Learning (CIL), which is more in line with the practical application requirements of real-world scenarios. However, existing CL methods often suffer from catastrophic forgetting (CF) and higher computing costs due to complex algorithm designs, limiting their practical use. Our proposed framework overcomes these limitations by achieving superior average accuracy and time-space efficiency, bridging the performance gap between CL and classical machine learning. Specifically, we adopt an independent Generated Kernel Density Estimation (GKDE) model for each CL task. During the testing stage, the GKDEs utilize a self-reported max probability density value to determine which one is responsible for predicting incoming test instances. A GKDE-based learning objective can ensure that samples with the same label are grouped together, while dissimilar instances are pushed farther apart. Extensive experiments conducted on multiple CL datasets validate the effectiveness of our proposed framework. Our method outperforms popular CL approaches by a significant margin, while maintaining competitive time-space efficiency, making our framework suitable for real-world applications. Code will be available at https://github.com/xxxx/xxxx.
\end{abstract}

==> sec/1_intro1.tex <==
\section{Introduction}
\label{intro}
Although current artificial intelligence systems~\cite{ResNet, ViT} have achieved promising performance on many tasks thanks to their excellent feature extraction abilities, the performance can drop dramatically when the models are tested on unseen data in new environments. \emph{Catastrophic forgetting}~\cite{catastrophic, catastrophic2} refers to the phenomena that previously learned knowledge is forgotten while learning new tasks under Continual learning (CL)~\cite{survey1, survey2, survey3, CL_CIL1} settings. Online CL is designed to learn continuously from a non-stationary data stream while adapting to new instances, mimicking the human general intelligence. In this paper, we focus on the class-incremental learning (CIL) in the online CL mode~\cite{online_survey, onlineCL1, onlineCL2, ASER}, which means the model learns incrementally labels in a sequence of tasks from a single-pass data stream and cannot access task information at inference.

Among the current online CL models~\cite{ASER, SCR, DVC, online_pro_accum, ER, ER_AML, onlineCL1}, replay-based methods~\cite{ER,  SCR, OCM, MIR, DVC} exhibit promising performance by storing part of training samples to facilitate upcoming task learning. Parameter-isolation methods train and protect a sub-network for each task\cite{Mallya2017packnet,abati2020conditional,von2019continual_hypernet,rajasegaran2020itaml,hung2019compact,henning2021posterior}, e.g., HAT \cite{Serra2018overcoming} and SupSup~\cite{supsup2020}, achieving excellent results. Though significant efforts have been devoted to the online CL field, there still exists some obstacles prohibiting the CL model from being deployed for practical application. Firstly, the training and the inference efficiency of the current CL models are relatively low due to complicated CL network design and additional memory usage to replay the previous samples. Secondly, there is a large performance gap between the popular CL methods and the classic machine learning algorithms. Lastly, the feature presentation of the current methods can not capture the causal factors to make predictions and thus have a low generalization ability. 

To solve the above problems, we propose a kernel density estimation (KDE) based learning framework with newly designed training objectives to replace the classic cross entropy loss, which is build upon elementary Residual or Transformer Network~\cite{ResNet, ViT}
with a simple linear projection head. The training of our method is efficient as no complicated network designs are employed and no replay memory is used. Our next inspiration is come from the no free lunch theorem~\cite{LamL09}, which states that no single best algorithm can solve all tasks, let alone the unseen and free-changing test samples in the future tasks and the robustness of an algorithm is dependent on the specific problem being solved. Each particular model is biased towards a kind of data distribution, and considering all data slices, the performance of all existing CL models are approaching the ERM~\cite{domainbed} or even inferior to the latter. Thus, we train an independent model for each task, and in the inference stage for a given test sample, all the models in the model bank can report their probability density value for the test instance, deciding which model is in charge of the current prediction. This mechanism make our model achieve state-of-the-art average accuracy, eliminating the performance gap with classic machine learning methods. For the last part, the feature representation in our model is aligned with probability density value, which enhances the causal factors and prohibits spurious features, leading to better model generalization. Extensive experiments on three CL datasets confirms our proposed method.

The contributions are summarized as follows. 

\begin{enumerate}[leftmargin=12pt, itemsep=0pt, topsep=0pt, partopsep=0pt, noitemsep]
	\item[1)] We design a density distribution-based learning framework to address the online CL problem, which achieves state-of-the-art performance and exhibits higher training efficiency and lower memory cost. 
	\item[2)] We build a model bank to store the trained GKDE model for each task and in the test stage, each model can recommend itself for processing the incoming test instances with self-reported distance metric. The task identifier prediction and within task class classification can be incorporated and achieve excellent performance. 
	\item[3)] The feature representation of our method is aligned with probability density value, which shows better model generalization in prediction unseen test samples, which is more suitable to solving online CL problems.
\end{enumerate}




==> sec/1_intro_-_____.tex <==
\section{Introduction}
\label{intro}
Although current artificial intelligence systems \cite{ResNet, ViT} have achieved promising performance on many tasks, their performance can significantly degrade when tested on unseen data in new environments. This phenomenon, known as \emph{catastrophic forgetting} (CF) \cite{catastrophic, catastrophic2}, occurs when previously learned knowledge is forgotten while learning new tasks in Continual Learning (CL) settings \cite{survey1, survey2, survey3, CL_CIL1}. Online CL aims to continuously learn from a non-stationary data stream, adapting to new instances and mimicking human general intelligence. In this paper, we specifically focus on Class Incremental Learning (CIL) in the online CL mode \cite{online_survey, onlineCL1, onlineCL2, ASER}. In CIL, the model incrementally learns labels in a sequence of tasks from a single-pass data stream and does not have access to task information during inference.

Among the current online CL models \cite{ASER, SCR, DVC, online_pro_accum, ER, ER_AML, onlineCL1}, replay-based methods \cite{ER, SCR, OCM, MIR, DVC} have shown promising performance by storing a portion of training samples to facilitate learning of upcoming tasks. Parameter-isolation methods, such as HAT \cite{Serra2018overcoming} and SupSup \cite{supsup2020}, train and protect a sub-network for each task, achieving excellent results \cite{Mallya2017packnet, abati2020conditional, von2019continual_hypernet, rajasegaran2020itaml, hung2019compact, henning2021posterior}. Despite the significant efforts dedicated to the field of online CL, several obstacles hinder the deployment of CL models for practical applications. Firstly, the training and inference efficiency of current CL models are relatively low due to complex network designs and additional memory usage required for replaying previous samples. Secondly, there exists a substantial performance gap between popular CL methods and classic machine learning (ML) algorithms. Lastly, the feature representation employed by current methods fails to capture causal factors for making predictions, resulting in limited generalization ability. Addressing these challenges is crucial to advancing the practical application of CL models. This paper aims to overcome these obstacles by proposing an efficient and high-performing CL framework that incorporates causal factor capture for improved generalization ability.

We propose a density distribution-based learning framework, named GKDE, to address the online CL issues. This framework replaces the traditional cross entropy loss with a probability density-based learning objective and is built upon elementary Residual or Transformer Networks \cite{ResNet, ViT} with a simple linear projection head. Our method is both time and space efficient, thanks to its simple network structure and straightforward training procedure. Inspired by the \emph{No Free Lunch} theorem \cite{LamL09}, which states that no single algorithm can solve all tasks optimally, we acknowledge that each model is biased towards a specific data distribution. Considering the diverse and evolving nature of future tasks and the limitations of existing CL models, we train an independent model for each task. During the inference stage, all models in the Model Bank (MB) report their probability density values for a given test sample, allowing us to determine which one is responsible for the current prediction. This mechanism enables our model to achieve state-of-the-art average accuracy, eliminating the performance gap with classic ML. In our model, the feature representation is aligned with the probability density value, enhancing the capture of causal factors while discouraging the influence of spurious features. This leads to improved model generalization. Extensive experiments conducted on three CL datasets validate the effectiveness of our proposed method. 

The contributions are summarized as follows. 

\begin{enumerate}[leftmargin=12pt, itemsep=0pt, topsep=0pt, partopsep=0pt, noitemsep]
	\item A unique density-based learning framework is proposed, referred to as GKDE, to tackle the challenges of CL by improving feature representations. This framework achieves state-of-the-art average accuracy, which solves the DF issue and bridges the performance gap between CL and classical ML.
	\item Our method is both time and space efficient, thanks to its simple network structure and straightforward training procedure. Compared to peer methods, our method is more suitable to be deployed for practical applications. 
	\item The feature representation of our method is aligned with  probability density values, leading to enhanced model generalization when predicting unseen test samples. This improvement is verified through experiments in three CL datasets with higher average accuracy.
\end{enumerate}

==> sec/2_related_-_____.tex <==
\section{Related Works}
\textit{Parameter-isolation methods} protect some network parameters for each task \cite{Mallya2017packnet,abati2020conditional} in the training stage, such as HAT \cite{Serra2018overcoming} and SupSup~\cite{supsup2020}, overcoming CF issue effectively. Other methods~\cite{PNN, para-iso1, pathNet} avoid forgetting by dynamically allocating parameters or modifying the architecture of the network. A limitation of the above methods is that the task-ids must be provided for test instances. To differentiate between tasks, \textit{Orthogonal projection} methods learn each task in an orthogonal space to reduce task confusion~\cite{lin2022beyond}. Different from the above methods, the GKDE learning framework can achieve task-id identification (TP) and within task prediction (WP) at the same time, and transform the CL into a classic machine learning problem.

\textit{Replay-based methods}~\cite{ER, MIR, GSS, AGEM, DER++, GDumb} maintain  a memory buffer which stores some samples of prior tasks. These methods are most popular due to their simplicity yet efficiency. Experience Replay~\cite{ER} randomly samples from the buffer. MIR~\cite{MIR} retrieves memory bank instances by comparing the interference of losses. Furthermore, in the online setting, ASER~\cite{ASER} proposes a buffer management algorithm to optimize the sampling process. OCM~\cite{OCM} prevents forgetting via mutual information maximization. Unlike these methods, our work do not need memory bank and rethinks the catastrophic forgetting from a new probability density learning perspective, and proposes to learn representative and discriminative features through KDE framework.

\textit{Prototypes based methods}~\cite{iCaRL, SCR, protoAug} aim to address catastrophic forgetting by incorporating prototypes. Recent works~\cite{online_pro_accum, onpro} solve CL problems by computing class prototypes via mean update criteria. However, regardless of whether momentum update or mean update is used, the accumulation of previous features as prototypes may hinder future learning. This is because the features learned for old classes may not be effective for distinguishing new labels. In contrast, the proposed GKDE framework leverages the training data by constructing probability density distributions for each class instead of prototypes. This approach accurately captures class information from the training data and is better suited for online CL.

\textit{Contrastive learning based methods} such as~\cite{SCR, ER_AML, OCM, Co2L, online_pro_accum} are following the self-supervised learning~\cite{SimCLR}, where the generalized features can boost the online CL performance. An early work~\cite{ssl4onlineCL} analyzes and confirms this impact. In this paper, feature embeddings based on the training samples with some uncertainties are generated as feature randomness is beneficial to enhance model generalization, which is confirmed by \cite{li2022uncertainty}. However, different from CL, the training efficiency of the GKDE framework is higher as complex augmentation and negative sampling in CL are not required.



==> sec/3_method_-_____.tex <==
\section{Proposed Method}

Fig.~\ref{fig:framework} presents the illustration of the proposed framework.
In the first section,  we start by explaining our overall architecture. Then, we describe the definition of the GKDE, the training objective, and the theoretical analysis of the method successively. 

\subsection{Overall Architecture}
In the inference stage of CIL for an instance without task id, the prediction probability is the product of two produced probabilities: \textit{WP} and \textit{TP}, 
\begin{align}
	\label{tp_and_wp}
	\mathbf{P}(X_{k,j} | x)
	&= \mathbf{P} (X_{k,j} | x, k) \mathbf{P}(X_{k} | x), 
\end{align}
where $X_{k,j}$ represents instances belonging to task $k$ and class label $j$. When it comes to a test instance $x$, we compute two probabilities using the same GKDE framework. The first probability, located on the right-hand side (RHS), represents WP. The second probability, represents TP. It is worth noting that our method stands out from others in that both probabilities are computed using a single GKDE framework. In contrast, alternative methods often rely on separate models or subnetworks to calculate these probabilities. By unifying the computation within a single framework, our approach offers a more streamlined and efficient solution. 

\input{fig/Framework.tex}

The proposed method is depicted in Fig.~\ref{fig:framework}. The backbone network, such as ResNet or Transformer, serves as the feature extraction unit without any modifications. A projection head is employed to generate $d$-dimensional probability density values, which replaces the traditional linear classification layer and cross entropy loss. In our approach, the class in each task, such as Giraffe or Elephant in Fig.~\ref{fig:framework}, is represented by a probability density function (PDF). The GKDE training objective is designed to bring samples with the same label closer together in higher probability regions, while pushing dissimilar samples, shown in the top right of Fig.~\ref{fig:framework}, further away from this ambiguous region. During the inference stage, the probability of a test sample is computed against each PDF in the Model Bank. By selecting the PDF with the highest probability, the correct model is recommended, enabling high-performance WP.

\subsection{Generative Kernel Density Estimation}
In this paper, we consider the dataset distribution represented as $(\boldsymbol{X}, Y)$, where $\boldsymbol{X}$ represents images, $\boldsymbol{Z}$ the features, and $Y$ the ground truth labels. $\boldZ = (Z_1, Z_2, \dots Z_d)^T \in \mathbb{R}^d$ is the $d$-dimensional features extracted by backbones and $Y \in \mathbb{R}$ is the target. In contrast to other methods, we use the GKDE for each class in the feature embedding space to align $\boldsymbol{Z}$ with PDFs and measure the distribution shifts between the test sample and each PDF in our Model Bank. By aggregating instances of each category into a compact PDF, we can effectively measure and predict samples in the unknown test distribution, achieving both TP and WP simultaneously. 

Formally, online CIL processes a continuous sequence of tasks from a single-pass data stream $\mathfrak{D}=\left\{\mathcal{D}_1, \ldots, \mathcal{D}_T \right\} $, where $\mathcal{D}_t = \left\{ x_{i}, y_{i} \right\} ^{N_t}_{i=1} $ is the training set of task $t$, and $T$ is the overall number of tasks. Training Set $\mathcal{D}_t$ contains $N_t$ samples, $y_{i}$ is the label of sample $x_{i}$ and $y_{i} \in \mathcal{C}_t$, where $\mathcal{C}_t$ is the label set of task $t$ and the labels in each task are different. The objective of online CIL is to achieve accurate predictions for incoming instances, regardless of whether they belong to an older or current task.

In this paper, $\phi_\theta(\cdot)$ represents the feature extractor parameterized by $\theta$, and $f_\psi(\cdot)$ represents the projection component for the GKDE framework, where $\psi$ is the parameter to be learned. The features generated by $\phi_\theta(\cdot)$ are further transformed into a $d$-dimensional feature space denoted as $\boldZ$. For training samples in the embedding space $\mathbf{z}_1,\ldots,\mathbf{z}_n$ in $\mathbb{R}^d$, the GKDE is evaluated at $\mathbf{x} \in \mathbb{R}^d$:
\begin{align}
	\label{general}
	\hat{k}(\mathbf{z};\mathbf{H}):=\frac{1}{n|\mathbf{H}|^{1/2}}\sum_{i=1}^nK\left(\mathbf{H}^{-1/2}(\mathbf{z}-\mathbf{z}_i)\right),
\end{align}
where $K$ is a multi-variate kernel and $\mathbf{H}$ is a bandwidth matrix, which is $d \times d$ symmetric and positive definite. For the sake of simplicity, we consider a Gaussian function as the kernel $K$ in our training objective, where $\boldsymbol{\mu}$ and $\boldsymbol{\Sigma}$ are computed from the samples of a specific class in a task. The bandwidth matrix $\mathbf{H}$ is replaced by a scalar value $h$, which is applied to each dimension. As a result, the GKDE can be further simplified as: 
\begin{equation}
	\label{specific}
	\hat{k}(\mathbf{z},h) = \frac{1}{nh^d} \sum_{i=1}^{n} K(\frac{\mathbf{z} - {\mathbf{z}}_i}{h}) = \frac{1}{n} \sum_{i=1}^{n} K_h (\mathbf{z} - {\mathbf{z}}_i)\,
\end{equation}
In Equation~\ref{general} and Equation~\ref{specific}, $\mathbf{z}$ represents the embedding feature of a training sample. On the other hand, $\mathbf{z_i}$ serves as the anchor point for a specific PDF to facilitate the computation of GKDE. These anchor points are randomly generated using the original training features and the bandwidth. We sample $n$ feature embeddings for each class of a specific task to act as anchor points. Therefore, unlike replay-based CL, our framework does not require storing any training samples. Instead, feature embeddings are generated based on the training samples, incorporating some uncertainties. This feature randomness is beneficial for enhancing model generalization, as confirmed by \cite{li2022uncertainty}. The specific value of the sample size $n$ will be discussed in the experimental section.

\subsection{The Training Objective}
In this part, we design our learning objective to serve as the training loss to replace the cross entropy and guide the network training process. Let’s denote by $k^{j=y}$ as the conditional PDF of $\mathbf{Z}|Y=j$. $\pi_j$ is the value of the probability mass function of  Y at $j$, i.e., $\mathbb{P}[Y=j]=\pi_j$, for $j=1,\ldots, m$, and $m$ is the number of distinct labels in the training set of a specific task. Estimating the class probabilities $\pi_j$ is based on their relative frequencies $\hat{\pi}_j:=\frac{n_j}{n}$, where $n_j:=\#\{i=1,\ldots,n:Y_i=j\}$. 
Therefore, the learning objective for the $j_{th}$ class is designed as:
\begin{align}
	\label{loss}
	\mathcal{L}(\mathbf{z})=-\hat{\pi}_j\hat{k}^{j = y}(\mathbf{z})+ \sum_{j=1,j \neq y}^m \hat{\pi}_j\hat{k}^{j \neq y}(\mathbf{z}),
\end{align}
where $\mathbf{z}$ is the embedding feature of a training sample and $\mathbf{y}$ is its corresponding label. In Equation.~\ref{loss}, there are two components and the first one aims to maximize the probability as the sample $\mathbf{z}$ belongs to the PDF $\hat{k}^{j = y}(\mathbf{z})$. While for the second term, we should minimize the probability as the training feature $\mathbf{z}$ has nothing to do with the PDF $\hat{k}^{j \neq y}(\mathbf{z})$. Guided by this learning objective, samples with the same label are encouraged to be grouped together in a region of higher probability, while dissimilar samples are pushed away to a region of marginal probability. Additionally, considering the training feature $\mathbf{z}$, the loss of the GKDE can be expressed in terms of the learnable parameters $\mathbf{\theta}$ and $\mathbf{\psi}$.
\begin{align}
	\label{loss_final}
	\begin{aligned}
		\mathcal{L}(\mathbf{\theta},\mathbf{\psi}; \mathbf{z})&= -\hat{\pi}_j \sum_{i=1}^{n} K^{j = y}_h (\mathbf{z} - {\mathbf{z}}_i)\\
		&+ \hat{\pi}_j \sum_{j=1,j \neq y}^m \sum_{i=1}^{n} K^{j \neq y}_h (\mathbf{z} - {\mathbf{z}}_i)\\	
		&= -\hat{\pi}_j \sum_{i=1}^{n} K^{j = y}_h (\mathbf{f}_{\psi}(\mathbf{\phi}_{\theta}(\mathbf{x})) - \mathbf{z}_i)\\
		& +\hat{\pi}_j \sum_{j=1,j \neq y}^m \sum_{i=1}^{n} K^{j \neq y}_h (\mathbf{f}_{\psi}(\mathbf{\phi}_{\theta}(\mathbf{x})) - \mathbf{z}_i).
	\end{aligned}
\end{align}

In Equation.~\ref{loss_final}, $\mathbf{\phi}_{\theta}(\cdot)$ and $\mathbf{f}_{\psi}(\cdot)$ represent the feature extractor and the projection head, respectively. These can be implemented using models such as ResNet \cite{stable_learning} or Transformer \cite{transformer}, and they contain the trainable parameters $\theta$ and $\psi$. Here, $\mathbf{x}$ denotes the training sample and $\mathbf{z_i}$ represents the anchor feature in the $j_{th}$ PDF. Equation~\ref{loss_final} is utilized as a loss function in our framework. Since the probability values involved in the loss computation for each anchor are in logarithmic format, we apply a clipping operation to ensure the values are not less than a threshold $\gamma$. This clipping operation not only stabilizes the training process but also prevents the values from underflow during backpropagation.

In the testing stage, for each test instance, the task label is determined through the TP procedure.
\begin{align}
	\label{inference}
	\begin{aligned}
		\mathcal{T}= \mathop{\arg\max}\limits_{t} \mathop{\arg\max}\limits_{j} k_{j}^t(\mathbf{f}_{\psi}^t(\mathbf{\phi}_{\theta}^t(\mathbf{x}))),
	\end{aligned}
\end{align}
where $t$ represents the task index that has been previously trained and stored in the Model Bank. $j$ represents the class label within task $t$, and $\mathcal{T}$ denotes the predicted task ID.

For WP, to assign an observation $\mathbf{z}$ of $\mathbf{Z}$
to each of the classes of $\mathbf{Y}$ can be solved by maximizing the conditional probability:
\begin{align}
	\mathbb{P}[Y=j|\mathbf{Z}=\mathbf{z}]&=\frac{k_j^{\mathcal{T}}(\mathbf{z})\mathbb{P}[Y=j]}{k^{\mathcal{T}}(\mathbf{z})}\nonumber\\
	&=\frac{\pi_jk_j^{\mathcal{T}}(\mathbf{z})}{\sum_{j=1}^m \pi_jk_j^{\mathcal{T}}(\mathbf{z})},
\end{align}
where $\mathbf{z}$ is assigned to the most likely class $j$. 
\begin{align}
	\label{WP}
	k_{\mathrm{Bayes}}^{\mathcal{T}}(\mathbf{z}):=\arg\max_{j=1,\ldots,m} \pi_jk_j^{\mathcal{T}}(\mathbf{z}).	
\end{align}

According to Equation~\ref{inference}, we can achieve TP and select the correct model corresponding to $\mathcal{T}$. Subsequently, based on Equation~\ref{WP}, we can achieve the WP. Therefore, the procedure defined in Equation~\ref{tp_and_wp} for a test instance is implemented in an online CL fashion.

\subsection{Theoretical Analysis of the Model Generalizability}

The GKDE framework exhibits excellent generality even though the test instances have severe co-variate shift. In this part, we give some theoretical analysis of the model generality. In the training process, the derivatives of the GKDE loss w.r.t parameters $\theta$ and $\psi$ are updated in the backward propagation. For a PDF $k(\cdot):\mathbb{R}^d\longrightarrow\mathbb{R}$, its gradient $\mathrm{D}k(\mathbf{z}):\mathbb{R}^d\longrightarrow\mathbb{R}^d$ is defined as:

\begin{align}
	\mathrm{D}k(\mathbf{z}):=\begin{pmatrix}\frac{\partial k(\mathbf{z})}{\partial \mathbf{z_1}}\\\vdots\\\frac{\partial k(\mathbf{z})}{\partial \mathbf{z_d}}\end{pmatrix}.	
\end{align}

The Hessian of $k(\cdot)$ is:
\begin{align}
	\mathrm{H}k(\mathbf{z}):=\left(\frac{\partial^2 k(\mathbf{z})}{\partial \mathbf{z_i}\partial \mathbf{z_j}}\right),\quad i,j=1,\ldots,d.
\end{align}

To quantify the bias and variance of the function $k(\cdot)$, which is commonly used to assess the generalizability of machine learning models, we employ the $\mathrm{vec}$ operator to concatenate the columns of the Hessian matrix into a single vector for easy expression, similar to the Kronecker product $\mathrm{D}^{\otimes 2}:=\mathrm{D}\otimes\mathrm{D}$. By doing so, we obtain Eq.~\ref{bias_and_variance}, which provides a characterization of the bias and variance of the GKDE at the point $\mathbf{z}$.

\begin{align}
	\label{bias_and_variance}
	\begin{aligned}
		\mathrm{Bias}[\hat{k}(\mathbf{z};\mathbf{H})]&=\frac{1}{2}\mu_2(K)(\mathrm{D}^{\otimes2}k(\mathbf{z}))'\mathrm{vec}\,\mathbf{H}+o(\|\mathrm{vec}\,\mathbf{H}\|),\\
		\mathbb{V}\mathrm{ar}[\hat{k}(\mathbf{z};\mathbf{H})]&=\frac{R(K)}{n|\mathbf{H}|^{1/2}}k(\mathbf{z})+o((n|\mathbf{H}|^{1/2})^{-1}),
	\end{aligned}
\end{align}
where $R(K)=\int K(\mathbf{z})^2\,\mathrm{d}\mathbf{z}$ and $\mu_2(K):=\int \mathbf{z}^2 K(\mathbf{z})\,\mathrm{d}\mathbf{z}$. The detailed computation can be found in the Appendix A. 

Equation~\ref{bias_and_variance} provides a theoretical framework for understanding how the Gaussian Kernel Density Estimation (GKDE) achieves model robustness and generality. The bias term in Eq.~\ref{bias_and_variance} represents the training error of the GKDE, while the variance term reflects the test error resulting from model overfitting.

As the value of $\mathbf{H}$ increases, the bias term decreases, indicating decreased training errors and improved model robustness. On the other hand, the variance term serves as an indicator of sensitivity to overfitting. A high variance implies a decrease in model generality, which is dependent on the value of $k(\mathbf{z})$, and decreases as a factor of $(n|\mathbf{H}|^{1/2})^{-1}$. In the case of a specific task with multiple probability density functions (PDFs), the peripheral region of the distribution bears the brunt of conflicting with other PDFs. However, by assigning small values to $k(\mathbf{z})$ in higher dimensions, overfitting can be alleviated.

The choice of bandwidth $\mathbf{H}$ and embedding dimension plays a crucial role in striking a balance between bias and variance, which will be further analyzed in our experimental settings.




==> sec/4_experiment_-_____.tex <==
\section{Experiments}
\subsection{Experimental Setup}
\paragraph{Datasets.}
We use three image classification benchmark datasets, including \textbf{CIFAR-10}~\cite{cifar10_100}, \textbf{CIFAR-100}~\cite{cifar10_100}, and \textbf{TinyImageNet}~\cite{tinyImageNet}, to evaluate the performance of online CIL methods. 
Following~\cite{ASER, SCR, DVC}, we split CIFAR-10 into 5 disjoint tasks, where each task has 2 disjoint classes, 10,000 samples for training, and 2,000 samples for testing, and split CIFAR-100 into 10 disjoint tasks, where each task has 10 disjoint classes, 5,000 samples for training, and 1,000 samples for testing.
Following~\cite{OCM}, we split TinyImageNet into 100 disjoint tasks, where each task has 2 disjoint classes, 1,000 samples for training, and 100 samples for testing.
Note that the order of tasks is fixed in all experimental settings.

\paragraph{Baselines.}
We compare our with 13 baselines, including 10 replay-based online CL baselines: {AGEM}~\cite{AGEM}, {MIR}~\cite{MIR}, {GSS}~\cite{GSS}, {ER}~\cite{ER}, {GDumb}~\cite{GDumb}, {ASER}~\cite{ASER}, {SCR}~\cite{SCR}, {CoPE}~\cite{online_pro_ema}, {DVC}~\cite{DVC}, and {OCM}~\cite{OCM}; 3 offline CL baselines that use knowledge distillation by running them in one epoch: {iCaRL}~\cite{iCaRL}, {DER++}~\cite{DER++}, and PASS~\cite{protoAug}. Note that PASS is a non-exemplar method.

\paragraph{Evaluation metrics.}
We use Average Accuracy and Average Forgetting~\cite{ASER, DVC} to measure the performance of our framework in online CIL. Average Accuracy evaluates the accuracy of the test sets from all seen tasks, defined as $\text {Average Accuracy} =\frac{1}{T} \sum_{j=1}^T a_{T, j},$
where $a_{i, j}$ is the accuracy on task $j$ after the model is trained from task $1$ to $i$.
Average Forgetting represents how much the model forgets about each task after being trained on the final task, defined as
$\text { Average Forgetting } =\frac{1}{T-1} \sum_{j=1}^{T-1} f_{T, j}, 
\text { where } f_{i, j}=\max _{k \in\{1, \ldots, i-1\}} a_{k, j}-a_{i, j}.$

\paragraph{Implementation details.}
We use ResNet18~\cite{ResNet} and VIT~\cite{ViT} as the backbone $\phi_{\theta}$ respectively and a linear layer as the projection head $f_{\psi}$ like~\cite{SCR, OCM, Co2L}; the hidden dim $d$ in $f$ is a hyper-parameter, which will be increased from 16 to 128 incrementally and be verified in the experiments. No linear layer is employed as the classifier. We train the model with Adam optimizer and an initial learning rate of $5\times10^{-4}$ for all datasets. The weight decay is set to $1.0\times10^{-4}$. The batch size $N$ is set to 128, and no replay memory are used. 
We reproduce all baselines in the same environment with their source code and default settings. We report the average results across 15 runs for all experiments.

\subsection{Combating Catastrophic Forgetting}
\begin{figure*}
	\label{other}
	\centering
	\includegraphics[width=1.0\linewidth]{fig/old.pdf}
	\caption{$t$-SNE~\cite{tsne} visualizations of features learned from ER and OnPro on the test set of CIFAR-10. When learning new classes, ER suffers serious class confusion probably. While OnPro relieves this issue to some extent, however, after the task2 is accomplished, the class confusion problem still persist.
	}	
\end{figure*}

\begin{figure*}
	\label{tsne_motivation}
	\centering
	\includegraphics[width=1.0\linewidth]{fig/alltask.pdf}
	\caption{$t$-SNE~\cite{tsne} visualizations of features learned from the proposed GKDE framework and on the test set of CIFAR-10. As new tasks are incrementally added, and the classes are accommodating Bird, Cat, Deer, Dog, Frog, Horse, Ship and Truck sequentially, the Catastrophic Forgetting almost disappear and the gap between online CL and classic machine learning is almost closed.. 
	}

\end{figure*}

Catastrophic Forgetting is the primary problem in online CL since the model cannot capture sufficient representative features in the embedding  feature space due to the single-pass data stream. To illustrate  this issue, some state-of-the-art papers are depicted in Fig.2 and the $t$-SNE~\cite{tsne} visualization results for ER and OnPro\cite{onpro} on the test set of CIFAR-10, both of which adopt ($M=0.2k$) re-play memory. There are five tasks and each contains two classes in these setting. There exists serious class confusion in ER and OnPro after task 2 is added and features learned in task 1 are not discriminative for task 2, leading to task confusion and decreased performance in old classes. Namely, the Task Prediction (TP) cannot be achieved in these methods. Even the Within Task Prediction (WP) based on classic machine learning methods are far from satisfactory, for instance, in Task 2, the Cat and Bird classed are not well distinguished.

In Fig.3, as each task from 1 to 5 are added, our proposed GKDE framework performs unbelievably excellent. In Task 1, the Airplane and Automobile are perfectly separated, which surpass peer classic machine learning methods given the task id as ER and OnPro in Fig.~\ref{other}. As new tasks are incrementally added, and the classes are accommodating Bird, Cat, Deer, Dog, Frog, Horse, Ship and Truck sequentially, the Catastrophic Forgetting almost disappear. In the end, all the ten classes can be separated in the PDF feature space. To our best knowledge, no other online CL moethods can approach this performance, and the gap between online CL and classic machine learning is almost closed.

\paragraph{Performance of average accuracy.}

\begin{table*}[ht]
	\small
	\begin{center}
		\resizebox{\linewidth}{!}{
			\begin{tabular}{rrrrrrrrrrrr}
				\shline
				\multirow{2}{*}{Method}  & \multicolumn{3}{c}{CIFAR-10}   && \multicolumn{3}{c}{CIFAR-100}  && \multicolumn{3}{c}{TinyImageNet} \\ \cline{2-4}\cline{6-8}\cline{10-12}
				& $M=0.1k$   & $M=0.2k$   & $M=0.5k$     && $M=0.5k$     & $M=1k$     & $M=2k$     && $M=1k$      & $M=2k$ & $M=4k$   \\ \midrule
				iCaRL~\cite{iCaRL}    & 31.0\std{$\pm$1.2} & 33.9\std{$\pm$0.9} & 42.0\std{$\pm$0.9} && 12.8\std{$\pm$0.4}  & 16.5\std{$\pm$0.4}  & 17.6\std{$\pm$0.5} && 5.0\std{$\pm$0.3}   & 6.6\std{$\pm$0.4} & 7.8\std{$\pm$0.4} \\ 
				DER++~\cite{DER++}   & 31.5\std{$\pm$2.9} & 39.7\std{$\pm$2.7} & 50.9\std{$\pm$1.8} && 16.0\std{$\pm$0.6}  & 21.4\std{$\pm$0.9}  & 23.9\std{$\pm$1.0} && 3.7\std{$\pm$0.4} & 5.1\std{$\pm$0.8} & 6.8\std{$\pm$0.6} \\ 
				PASS~\cite{protoAug}    & 33.7\std{$\pm$2.2} & 33.7\std{$\pm$2.2} & 33.7\std{$\pm$2.2} && 7.5\std{$\pm$0.7}  & 7.5\std{$\pm$0.7}  & 7.5\std{$\pm$0.7} && 0.5\std{$\pm$0.1}   & 0.5\std{$\pm$0.1} & 0.5\std{$\pm$0.1} \\ 
				\hline
				AGEM~\cite{AGEM}    & 17.7\std{$\pm$0.3} & 17.5\std{$\pm$0.3} & 17.5\std{$\pm$0.2} && 5.8\std{$\pm$0.1}  & 5.9\std{$\pm$0.1}  & 5.8\std{$\pm$0.1} && 0.8\std{$\pm$0.1}   & 0.8\std{$\pm$0.1} & 0.8\std{$\pm$0.1} \\ 
				GSS~\cite{GSS}     & 18.4\std{$\pm$0.2} & 19.4\std{$\pm$0.7} & 25.2\std{$\pm$0.9} && 8.1\std{$\pm$0.2}  & 9.4\std{$\pm$0.5}  & 10.1\std{$\pm$0.8} && 1.1\std{$\pm$0.1}   & 1.5\std{$\pm$0.1} & 2.4\std{$\pm$0.4} \\ 
				ER~\cite{ER}      & 19.4\std{$\pm$0.6} & 20.9\std{$\pm$0.9} & 26.0\std{$\pm$1.2} && 8.7\std{$\pm$0.3}  & 9.9\std{$\pm$0.5}  & 10.7\std{$\pm$0.8} && 1.2\std{$\pm$0.1}   & 1.5\std{$\pm$0.2} & 2.0\std{$\pm$0.2} \\ 
				MIR~\cite{MIR}     & 20.7\std{$\pm$0.7} & 23.5\std{$\pm$0.8} & 29.9\std{$\pm$1.2} && 9.7\std{$\pm$0.3}  & 11.2\std{$\pm$0.4}  & 13.0\std{$\pm$0.7} && 1.4\std{$\pm$0.1}   & 1.9\std{$\pm$0.2} & 2.9\std{$\pm$0.3} \\ 
				GDumb~\cite{GDumb}   & 23.3\std{$\pm$1.3} & 27.1\std{$\pm$0.7} & 34.0\std{$\pm$0.8} && 8.2\std{$\pm$0.2}  & 11.0\std{$\pm$0.4}  & 15.3\std{$\pm$0.3} && 4.6\std{$\pm$0.3}   & 6.6\std{$\pm$0.2} & 10.0\std{$\pm$0.3} \\ 
				ASER~\cite{ASER}   & 20.0\std{$\pm$1.0} & 22.8\std{$\pm$0.6} & 31.6\std{$\pm$1.1} && 11.0\std{$\pm$0.3}  & 13.5\std{$\pm$0.3}  & 17.6\std{$\pm$0.4} && 2.2\std{$\pm$0.1}   & 4.2\std{$\pm$0.6} & 8.4\std{$\pm$0.7} \\ 
				SCR~\cite{SCR}     & 40.2\std{$\pm$1.3} & 48.5\std{$\pm$1.5} & 59.1\std{$\pm$1.3} && 19.3\std{$\pm$0.6}  & 26.5\std{$\pm$0.5}  & 32.7\std{$\pm$0.3} && 8.9\std{$\pm$0.3}   & 14.7\std{$\pm$0.3} & 19.5\std{$\pm$0.3} \\ 
				CoPE~\cite{online_pro_ema}  & 33.5\std{$\pm$3.2} & 37.3\std{$\pm$2.2} & 42.9\std{$\pm$3.5} && 11.6\std{$\pm$0.7}  & 14.6\std{$\pm$1.3}  & 16.8\std{$\pm$0.9} && 2.1\std{$\pm$0.3}   & 2.3\std{$\pm$0.4} & 2.5\std{$\pm$0.3} \\
				DVC~\cite{DVC} & 35.2\std{$\pm$1.7}  & 41.6\std{$\pm$2.7} & 53.8\std{$\pm$2.2} &&  15.4\std{$\pm$0.7} & 20.3\std{$\pm$1.0} & 25.2\std{$\pm$1.6} && 4.9\std{$\pm$0.6} &  7.5\std{$\pm$0.5} & 10.9\std{$\pm$1.1} \\ 
				OCM~\cite{OCM} & 47.5\std{$\pm$1.7}  & 59.6\std{$\pm$0.4} & 70.1\std{$\pm$1.5} && 19.7\std{$\pm$0.5} & 27.4\std{$\pm$0.3} & 34.4\std{$\pm$0.5} && 10.8\std{$\pm$0.4} & 15.4\std{$\pm$0.4} & 20.9\std{$\pm$0.7} \\ 
				OnPro~\cite{onpro} & 57.8\std{$\pm$1.1}  & 65.5\std{$\pm$1.0} & 72.6\std{$\pm$0.8} && 22.7\std{$\pm$0.5} & 30.0\std{$\pm$0.3} & 35.9\std{$\pm$0.5} && 11.9\std{$\pm$0.4} & 16.9\std{$\pm$0.4} & 22.1\std{$\pm$0.7} \\ 
				\hline
				\frameworkName (\textbf{ResNet-18}) & \multicolumn{3}{c}{90.6\std{$\pm$1.8}} && \multicolumn{3}{c}{78.54\std{$\pm$2.3}} && \multicolumn{3}{c}{82.35\std{$\pm$2.8}}
				\\ 
				\frameworkName (\textbf{VIT}) & \multicolumn{3}{c}{99.25\std{$\pm$0.8}} && \multicolumn{3}{c}{92.88\std{$\pm$1.9}} && \multicolumn{3}{c}{99.10\std{$\pm$1.2}}
				\\ 
				\shline
			\end{tabular}
		}
	\end{center}
	\caption{Average Accuracy~(higher is better) on three benckmark datasets. The baseline methods with different memory bank sizes $M$ exhibit different results. Our method does not need memory to store training samples but requires some generated embedding features, which will be analyzed in the next subsection, All results are the average and standard deviation of 15 runs.}
	\label{tab:acc}
\end{table*}

Table~\ref{tab:acc} lists the results of average accuracy of some baseline methods with different memory bank sizes ($M$) on three benchmark datasets. Our framework outperforms all baselines on three datasets to a new level, which almost closes the online CL problem. Remarkably, the performance improvement is achieved when the memory bank is not used for online CL. For example, compared to the peer methods which employ training samples from at least 100 to 4000, our method do not store any training samples and the GKDE framework just memorizes $n$ $d$-dimensional PDFs which are randomly generated based on training samples ($d$ usually from 16 to 128 and $d$ from 16 500 to 3000). Compared to baselines that use knowledge distillation (iCaRL, DER++, PASS, OCM) and prototypes (PASS, CoPE, OnPro), our framework exhibits a strong advantage and is more suitable for online CL. The baselines perform poorly on CIFAR-100 and TinyImageNet due to a dramatic increase in the number of tasks. In contrast,  our method's performance will not fluctuate as more tasks are added. The Average Forgetting of our method is nearly approaching to zero on three benchmark datasets. The results confirm that catastrophic forgetting issue is well addressed. All the Average Forgetting are omitted here due to limited space and please refer to OnPro. 

\begin{figure}[t]
	\label{incrementalAcc}
	\centering
	\begin{subfigure}[t]{3.0in}
		\centering
		\includegraphics[width=2.8in]{fig/cifar10.pdf}
		\caption{Top 1 Acc and Recall against the PDFs of Art}
	\end{subfigure}
	\\
	\begin{subfigure}[t]{3.0in}
		\centering
		\includegraphics[width=2.8in]{fig/cifar100.pdf}
		\caption{Top 1 Acc and Recall against the PDFs of Sketch}
	\end{subfigure}	
	\caption{Average incremental accuracy comparison between the GKDE and the baseline methods in the {test set} of CIFAR-10 and CIFAR-100. As our method can achieve TP with 100\% accuracy, thus the disastrous forgetting issue is removed. While the baseline methods are suffering from severe forgetting as new tasks are added. The GKDE framework based on VIT structure achieves excellence performance in the WP, and even the GKDE based on RestNet18 has an obvious edge over baseline methods. }
	\label{fig:fourfigures}
\end{figure}

\paragraph{How the performance changes as new tasks are added.}
We evaluate the average incremental performance~\cite{DER++, DVC} on CIFAR-10 ($M=0.1k$) and CIFAR-100 ($M=0.5k$), which indicates the accuracy over all seen tasks at each incremental step. 
Fig.~\ref{incrementalAcc} shows that \frameworkName achieves better accuracy and effectively removes forgetting while the performance of most baselines degrades rapidly with the arrival of new classes. As our method can achieve TP with 100\% accuracy, thus the disastrous forgetting issue is removed. While the baseline methods are suffering from severe forgetting as new tasks are added. The GKDE framework based on VIT structure achieves excellence performance in the WP, and even the GKDE based on RestNet18 has an obvious edge over baseline methods.

\begin{figure}
	\label{bandwidth}
	\centering
	\includegraphics[width=2.9 in,height=2.6 in]{fig/bandwith1.pdf}
	\caption{Bandwidth and Embedding dimmention Effects.When the embedding dimensions are fewer than 4, the framework exhibits signs of under-fitting, and there is minimal improvement as the dimension increases to 32 or beyond. The bandwidth parameter is a scalar value, and when it is below 0.1, the performance becomes unstable and leads to lower accuracy. Conversely, when the bandwidth exceeds 2.0, the framework's performance significantly deteriorates.}
\end{figure}


\paragraph{How the embedding dimension and bandwidth affect the performance.}
The embedding dimension and bandwidth play a key role in defining the GKDE function, thus in this part we validate how they affect the performance. To find the optimal parameter combination, we performed a grid search over the embedding dimensions of 2, 4, 8, 16, 32, and bandwidth values of 0.1, 1, 2, 3, 4, 5, and 6, which are illustrated in Fig.5. When the embedding dimensions are fewer than 4, the framework exhibits signs of under-fitting, and there is minimal improvement as the dimension increases to 32 or beyond. The bandwidth parameter is a scalar value, and when it is below 0.1, the performance becomes unstable and leads to lower accuracy. Conversely, when the bandwidth exceeds 2.0, the framework's performance significantly deteriorates. Based on the results of the grid search, we have selected dimension 32 and bandwidth 0.5 for CIFAR10. For CIFAR100 and TinyImageNet, we have opted for dimension 64 and bandwidth 0.2.

\paragraph{How the sample size affect model performance and time-space efficiency.}
For each class in the task, the GKDE framework samples a certain number of embedding features. In order to assess the impact of the sample size on model performance and efficiency, we experimented with various values ranging from 100 to 3000. Our findings indicate that a sample size of 500 yields the best results for CIFAR10, while for CIFAR100 and TinyImageNet, a sample size of 1500 is the optimal choice. Interestingly, increasing the sample size beyond these values does not lead to further performance improvements. Instead, it negatively affects the time and space efficiency during both the training and inference stages of the framework. For the memory usage in CIFAR10, our GKDE framework requires only one quarter of the memory compared to replay-based methods. Specifically, we need 500 samples * 32 dimensions (bytes) for each class, while the replay-based methods require a minimum of 200 * 32 * 32 * 3 bytes to store the original images. Regarding training efficiency, as shown in Fig. 6, we compared the GKDE framework with peer methods. Our method achieves impressive training time results, completing 5 tasks with 10 epochs per task in approximately 1 minute. Each epoch runs in just 1.5 seconds. Notably, the GKDE framework demonstrates significantly superior training efficiency compared to other peer methods, surpassing them by a large margin.

\begin{figure}
	\label{efficieny}
	\centering
	\includegraphics[width=2.9 in,height=2.6 in]{fig/time.pdf}
	\caption{Training Time Efficiency Comparison. Our method achieves impressive training time results, completing 5 tasks with 10 epochs per task in approximately 1 minute. Each epoch runs in just 1.5 seconds.}
\end{figure}


==> sec/5_discussion.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.

==> sec/6_conclusion.tex <==
\section{Conclusion}

In this paper, we introduce a density distribution-based learning framework for addressing the challenges of online CL. Our method strategically groups samples with the same label into high-density regions, while simultaneously pushing dissimilar samples apart. This approach leads to superior average accuracy with enhanced model generalization, outperforming existing peer methods by a substantial margin and effectively removing the issue of Disastrous Forgetting. Additionally, our proposed methods demonstrate commendable space-time efficiency during both the training and testing stages, making our method more suitable for real applications.
